On Memory System Design for Stochastic Computing

Growing uncertainty in design parameters (and therefore, in design functionality) renders stochastic computing particularly promising, which represents and processes data as quantized probabilities. However, due to the difference in data representation, integrating conventional memory (designed and optimized for non-stochastic computing) in stochastic computing systems inevitably incurs a significant data conversion overhead. Barely any stochastic computing proposal to-date covers the memory impact. In this paper, as the first study of its kind to the best of our knowledge, we rethink the memory system design for stochastic computing. The result is a seamless stochastic system, StochMem, which features analog memory to trade the energy and area overhead of data conversion for computation accuracy. In this manner StochMem can reduce the energy (area) overhead by up-to 52.8% (93.7%) at the cost of at most 0.7% loss in computation accuracy.

==> eval-sens.tex <==
\noindent As covered in Section~\ref{sec:pcm}, similar to MLC memories,
resistive analog memories may cause a
discrepancy between values read and written (i.e., stored). 
%when using a resistive analog memory, the data write and the data read steps 
%introduce inaccuracy to the data. 
To quantify the output sensitivity of evaluated SC systems to this discrepancy,
we inject random Gaussian noise with zero mean and standard deviation of $\sigma_{cell}$ to the input images.
To this end, we sweep $\sigma_{cell}$ from 1\% up to 7\% (Table~\ref{tbl:sigma}).
%to mimic the inaccuracy of a real cell.


Fig.~\ref{fig:sens} shows the output sensitivity of the stochastic circuit
implementations to potential read-write discrepancy introduced by analog memory.
%introduced by an analog cell. 
The sensitivity for each circuit is evaluated by the \% average output error 
in processing the sample input images when they are degraded with different rates of $\sigma_{cell}$. 
%As can be seen in the figure, 
As Fig.~\ref{fig:sens} reveals, 
for all stochastic circuits and different stochastic input bitstream lengths
(over a range from 128 to 1024),
\% output error increases only very gracefully with $\sigma_{cell}$. 
This is due to the intrinsic tolerance of SC systems to errors in input data. 
For instance, 
%in the case of 
%processing the input image with the 
for {\it Robert}, when pixel intensities are represented
with stochastic streams of 1024-bits, the average output error remains
around 3.2\% in the worst case ($\sigma_{cell}$=7\%). This still is an
accurate-enough output 
%, which is still accurate to 
considering the error bounds expected for stochastic computation.

The vertical bars at around $\sigma_{cell}$=1.9\% in Fig.~\ref{fig:sens} capture the $\sigma_{cell}$
of the 8-level PCM design from IBM~\cite{IBM_PCM2016}.
%The inaccuracy of a pcm-based analog cell based on \cite{IBM_PCM2016} ($\sigma_{cell}$=1.9\%) is shown in 
%Figure~\ref{fig:sens} with a vertical red line on each plot. 
%Extracting the average output error rate of processing degraded 
%sample images with the same level of inaccuracy 
For this particular value of $\sigma_{cell}$, the average output error across all
SC circuits remains less than
%shows an error rate of less than 
2\%.
%for all implemented
%stochastic circuits. 
%This means that in the case of 
Therefore, we do not anticipate any sizable degradation in the accuracy of end
results, if a similar design to this PCM implementation is adapted
as analog memory in an SC system.
%of a 
%stochastic system the likely benefits of replacing the conventional digital memory
%with an analog memory can be gained while still produce high-quality results.     



    


